StaticGreedy: solving the scalability-accuracy dilemma in influence maximization

Influence maximization, defined as a problem of finding a set of seed nodes to trigger a maximized spread of influence, is crucial to viral marketing on social networks. For practical viral marketing on large scale social networks, it is required that influence maximization algorithms should have both guaranteed accuracy and high scalability. However, existing algorithms suffer a scalability-accuracy dilemma: conventional greedy algorithms guarantee the accuracy with expensive computation, while the scalable heuristic algorithms suffer from unstable accuracy. In this paper, we focus on solving this scalability-accuracy dilemma. We point out that the essential reason of the dilemma is the surprising fact that the submodularity, a key requirement of the objective function for a greedy algorithm to approximate the optimum, is not guaranteed in all conventional greedy algorithms in the literature of influence maximization. Therefore a greedy algorithm has to afford a huge number of Monte Carlo simulations to reduce the pain caused by unguaranteed submodularity. Motivated by this critical finding, we propose a static greedy algorithm, named StaticGreedy, to strictly guarantee the submodularity of influence spread function during the seed selection process. The proposed algorithm makes the computational expense dramatically reduced by two orders of magnitude without loss of accuracy. Moreover, we propose a dynamical update strategy which can speed up the StaticGreedy algorithm by 2-7 times on large scale social networks.

==> chpt.authors.tex <==

%\subtitle{[Extended Abstract]
%\titlenote{A full version of this paper is available as
%\textit{Author's Guide to Preparing ACM SIG Proceedings Using
%\LaTeX$2_\epsilon$\ and BibTeX} at
%\texttt{www.acm.org/eaddress.htm}}}
%
% You need the command \numberofauthors to handle the 'placement
% and alignment' of the authors beneath the title.
%
% For aesthetic reasons, we recommend 'three authors at a time'
% i.e. three 'name/affiliation blocks' be placed beneath the title.
%
% NOTE: You are NOT restricted in how many 'rows' of
% "name/affiliations" may appear. We just ask that you restrict
% the number of 'columns' to three.
%
% Because of the available 'opening page real-estate'
% we ask you to refrain from putting more than six authors
% (two rows with three columns) beneath the article title.
% More than six makes the first-page appear very cluttered indeed.
%
% Use the \alignauthor commands to handle the names
% and affiliations for an 'aesthetic maximum' of six authors.
% Add names, affiliations, addresses for
% the seventh etc. author(s) as the argument for the
% \additionalauthors command.
% These 'additional authors' will be output/set for you
% without further effort on your part as the last section in
% the body of your article BEFORE References or any Appendices.

% \numberofauthors{1} %  in this sample file, there are a *total*
% of EIGHT authors. SIX appear on the 'first-page' (for formatting
% reasons) and the remaining two appear in the \additionalauthors section.
%
%\author{
% You can go ahead and credit any number of authors here,
% e.g. one 'row of three' or two rows (consisting of one row of three
% and a second row of one, two or three).
%
% The command \alignauthor (no curly braces needed) should
% precede each author name, affiliation/snail-mail address and
% e-mail address. Additionally, tag each line of
% affiliation/address with \affaddr, and tag the
% e-mail address with \email.
%
% 1st. author
%\alignauthor
%Suqi Cheng~~~~~~Huawei Shen~~~~~~Junming Huang~~~~~~Guoqing Zhang~~~~~~Xueqi Cheng\\
       %\affaddr{Institute of Computing Technology, Chinese Academy of Sciences, Beijing, China}\\
       %\affaddr{Chinese Academy of Sciences}\\
       %\affaddr{Beijing, China}\\
       %\email{\{chengsuqi, shenhuawei, huangjunming, gqzhang, cxq\}@ict.ac.cn}
% 2nd. author
%\alignauthor
%Huawei Shen\\
       %\affaddr{Institute of Computing Technology}\\
       %\affaddr{Chinese Academy of Sciences}\\
       %\affaddr{Beijing, China}\\
       %\email{shenhuawei@ict.ac.cn}
% 3rd. author
%\alignauthor
%Junming Huang\\
       %\affaddr{Institute of Computing Technology}\\
       %\affaddr{Chinese Academy of Sciences}\\
       %\affaddr{Beijing, China}\\
       %\email{mail@junminghuang.com}
%\and  % use '\and' if you need 'another row' of author names
% 4th. author
%\alignauthor Guoqing Zhang\\
       %\affaddr{Institute of Computing Technology}\\
       %\affaddr{Chinese Academy of Sciences}\\
       %\affaddr{Beijing, China}\\
       %\email{gqzhang@ict.ac.cn}
% 5th. author
%\alignauthor Xueqi Cheng\\
       %\affaddr{Institute of Computing Technology}\\
       %\affaddr{Chinese Academy of Sciences}\\
       %\affaddr{Beijing, China}\\
       %\email{cxq@ict.ac.cn}
%}


% There's nothing stopping you putting the seventh, eighth, etc.
% author on the opening page (as the 'third row') but we ask,
% for aesthetic reasons that you place these 'additional authors'
% in the \additional authors block, viz.
%\additionalauthors{Additional authors: John Smith (The Th{\o}rv{\"a}ld Group,
%email: {\texttt{jsmith@affiliation.org}}) and Julius P.~Kumquat
%(The Kumquat Consortium, email: {\texttt{jpkumquat@consortium.net}}).}
%\date{30 July 1999} % Just remember to make sure that the TOTAL number of authors
% is the number that will appear on the first page PLUS the
% number that will appear in the \additionalauthors section.
